Three-Currency HJM for Brazilian Credit Markets

This paper develops a three-currency Heath-Jarrow-Morton framework in which corporate credit is treated as a separate economy, connected to the nominal and real economies through synthetic inflation and credit exchange rates. The framework produces a testable identity. Under joint no-arbitrage, the credit spread of an issuer expressed over the inflation-rateindexed risk-free curve equals the same issuer's credit spread expressed over the nominalrate-indexed risk-free curve plus the model-implied breakeven inflation forward at the same maturity. The identity holds within any single calibration of the framework. It is empirically falsifiable across two parallel corporate-bond segments of the same market, in a segmented market the two segments may price different corporate credit economies, and the gap between their implied corporate forwards measures the failure of the shared-credit-economy assumption. Applied to Brazilian debenture markets, the framework delivers a sharp empirical finding. Fifteen large issuers placed paper in both the CDI-indexed general-purpose segment and the IPCA-indexed infrastructure segment between January 2021 and February 2026. The within-issuer triangle residual at the 3-year tenor averages 640 basis points, with crosssectional standard deviation of 26 basis points across the 15 issuer means, and remains stable through both the 2021-2023 BCB tightening cycle and the 2024-2026 easing phase. A retail post-tax indifference benchmark anchored on Lei 12.431 closes the bulk of the residual. The remainder is consistent with institutional participation on the CDI side, contractual asymmetries between debentures with different use-of-proceeds restrictions, and segment-specific liquidity gaps.

==> tables/tab_bucket_sensitivity.tex <==
% Bucket-width sensitivity at the index aggregate level
\begin{tabular}{lrrr}
\toprule
Bucket specification & Mean $\Delta_{agg}$ (bp) & SD (bp) & Valid days \\
\midrule
Tight (±0.25 for 1/2/3y, ±0.5 for 5y) & -684.6 & 57.3 & 641 \\
Baseline (±0.5 for 1/2/3y, ±1.0 for 5y) & -685.0 & 78.8 & 1112 \\
Wide (±0.75 for 1/2/3y, ±1.5 for 5y) & -686.1 & 81.2 & 1270 \\
\bottomrule
\end{tabular}


==> tables/tab_correlation.tex <==
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & $N1$ & $N2$ & $N3$ & $R1$ & $R2$ & $S1$ & $S2$ \\
\midrule
$N1$ & 1.00 &  &  &  &  &  &  \\
$N2$ & -0.05 & 1.00 &  &  &  &  &  \\
$N3$ & -0.06 & -0.11 & 1.00 &  &  &  &  \\
$R1$ & 0.54 & 0.24 & -0.08 & 1.00 &  &  &  \\
$R2$ & -0.56 & 0.27 & 0.17 & 0.00 & 1.00 &  &  \\
$S1$ & -0.06 & -0.03 & 0.10 & -0.23 & 0.01 & 1.00 &  \\
$S2$ & 0.10 & 0.01 & -0.01 & 0.18 & -0.09 & 0.00 & 1.00 \\
\bottomrule
\end{tabular}

==> tables/tab_correlation_cdi.tex <==
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & $N1$ & $N2$ & $N3$ & $R1$ & $R2$ & $S1$ & $S2$ \\
\midrule
$N1$ & 1.00 &  &  &  &  &  &  \\
$N2$ & -0.05 & 1.00 &  &  &  &  &  \\
$N3$ & -0.06 & -0.11 & 1.00 &  &  &  &  \\
$R1$ & 0.54 & 0.24 & -0.08 & 1.00 &  &  &  \\
$R2$ & -0.56 & 0.27 & 0.17 & 0.00 & 1.00 &  &  \\
$S1$ & -0.06 & -0.03 & 0.10 & -0.23 & 0.01 & 1.00 &  \\
$S2$ & 0.10 & 0.01 & -0.01 & 0.18 & -0.09 & 0.00 & 1.00 \\
\bottomrule
\end{tabular}

==> tables/tab_correlation_ipca.tex <==
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & $N1$ & $N2$ & $N3$ & $R1$ & $R2$ & $S1$ & $S2$ \\
\midrule
$N1$ & 1.00 &  &  &  &  &  &  \\
$N2$ & -0.22 & 1.00 &  &  &  &  &  \\
$N3$ & -0.14 & -0.32 & 1.00 &  &  &  &  \\
$R1$ & 0.67 & -0.22 & -0.09 & 1.00 &  &  &  \\
$R2$ & -0.63 & 0.19 & 0.13 & -0.21 & 1.00 &  &  \\
$S1$ & 0.05 & 0.07 & -0.04 & -0.00 & -0.08 & 1.00 &  \\
$S2$ & -0.02 & -0.06 & -0.04 & 0.02 & -0.06 & -0.00 & 1.00 \\
\bottomrule
\end{tabular}

==> tables/tab_coverage.tex <==
% OOS coverage of 90% Gaussian prediction intervals (weekly)
\begin{tabular}{@{}lcccc@{}}
\toprule
& $\tau = 1$y & $\tau = 3$y & $\tau = 5$y & $\tau = 7$y \\
\midrule
$\Delta f^N$       & 94.5\% & 98.2\% & 92.7\% & 90.9\% \\
$\Delta f^R$       & 91.8\% & 94.5\% & 75.5\% & 69.1\% \\
$\Delta s^{CDI}$   & 85.5\% & 92.7\% & 90.9\% & n/a \\
\bottomrule
\end{tabular}


==> tables/tab_d5.tex <==
% D5 smoothness diagnostic: scale-invariant second difference
\begin{tabular}{llcccc}
\toprule
Curve & $\tau$ window & init.\ max & sim.\ p50 & sim.\ p95 & p95/init \\
\midrule
$fN$ & 0.25-2y & 0.1683 & 0.0971 & 0.4891 & 2.91 \\
$fN$ & 2-10y & 0.0413 & 0.0117 & 0.0385 & 0.93 \\
$fR$ & 0.25-2y & 1.1310 & 0.3442 & 3.6874 & 3.26 \\
$fR$ & 2-10y & 0.0097 & 0.0058 & 0.0076 & 0.79 \\
$fC$ & 0.25-2y & 0.1647 & 0.1744 & 0.5636 & 3.42 \\
$fC$ & 2-10y & 0.0201 & 0.0120 & 0.0401 & 1.99 \\
$sCDI$ & 0.25-2y & 0.2975 & 0.3192 & 0.6281 & 2.11 \\
$sCDI$ & 2-10y & 0.1838 & 0.0019 & 0.0108 & 0.06 \\
$sIPCA$ & 0.25-2y & 0.9340 & 0.3508 & 2.8340 & 3.03 \\
$sIPCA$ & 2-10y & 0.0357 & 0.0107 & 0.0418 & 1.17 \\
\bottomrule
\end{tabular}


==> tables/tab_full_params.tex <==
% Complete calibrated parameter set, two-model framing.
\begin{tabular}{llll}
\toprule
Block & Parameter & Value & Source \\
\midrule
Nominal (shared) & $a^N_1$ & -4902.64 & PCA \\
Nominal (shared) & $a^N_2$ & -1671.50 & PCA \\
Nominal (shared) & $a^N_3$ & 4164.37 & PCA \\
Nominal (shared) & $b_2$ & 0.730 & NLS \\
Nominal (shared) & $b_3$ & 3.436 & NLS \\
Real (shared) & $a^R_1$ & 3375.63 & PCA \\
Real (shared) & $a^R_2$ & 11125.86 & PCA \\
Inflation FX (shared) & $|\sigma_I|$ & 135.1 bp & IPCA realized \\
Model A (CDI$^+$) & $a^{S,A}_1$ & 732.02 & PCA \\
Model A (CDI$^+$) & $a^{S,A}_2$ & 3128.55 & PCA \\
Model A (CDI$^+$) & $c_2^A$ & 3.751 & NLS \\
Model A (CDI$^+$) & $|\sigma_J^A|$ & 80.7 bp & $\Delta s^{CDI}(\tau_{\min})$ realized \\
Model B (IPCA$^+$) & $a^{S,B}_1$ & 3075299.20 & PCA \\
Model B (IPCA$^+$) & $a^{S,B}_2$ & 1026538.54 & PCA \\
Model B (IPCA$^+$) & $c_2^B$ & 5.000 & NLS \\
Model B (IPCA$^+$) & $|\sigma_J^B|$ & 75.9 bp & $\Delta s^{IPCA}(\tau_{\min})$ realized \\
\bottomrule
\end{tabular}


==> tables/tab_params_Nominal.tex <==
% Estimated Nominal factor parameters.
\begin{tabular}{ll}
\toprule
Parameter & Estimate \\
\midrule
$a^{N}_1$ (bp/$\sqrt{\text{yr}}$) & -4902.64 \\
$a^{N}_2$ (bp/$\sqrt{\text{yr}}$) & -1671.50 \\
$a^{N}_3$ (bp/$\sqrt{\text{yr}}$) & 4164.37 \\
$b_2$ (yr$^{-1}$) & 0.730 \\
$b_3$ (yr$^{-1}$) & 3.436 \\
Parametric fit $R^2$ & 88.2\% \\
\bottomrule
\end{tabular}


==> tables/tab_params_Real.tex <==
% Estimated Real factor parameters.
\begin{tabular}{ll}
\toprule
Parameter & Estimate \\
\midrule
$a^{R}_1$ (bp/$\sqrt{\text{yr}}$) & 3375.63 \\
$a^{R}_2$ (bp/$\sqrt{\text{yr}}$) & 11125.86 \\
$b_2$ (yr$^{-1}$) & 0.730 \\
$b_3$ (yr$^{-1}$) & 3.436 \\
Parametric fit $R^2$ & 99.5\% \\
\bottomrule
\end{tabular}


==> tables/tab_params_spread.tex <==
% Estimated spread factor parameters.
\begin{tabular}{ll}
\toprule
Parameter & Estimate \\
\midrule
$a^{S}_1$ (bp/$\sqrt{\text{yr}}$) & 3075299.20 \\
$a^{S}_2$ (bp/$\sqrt{\text{yr}}$) & 1026538.54 \\
$c_2$ (yr$^{-1}$) & 5.000 \\
Parametric fit $R^2$ & 97.8\% \\
\bottomrule
\end{tabular}


==> tables/tab_pca_Nominal.tex <==
% Nominal curve PCA: eigenvalues and variance explained.
\begin{tabular}{llll}
\toprule
Factor & Eigenvalue & % Variance & Cumulative % \\
\midrule
$N_1$ & 362588.5285 & 63.5\% & 63.5\% \\
$N_2$ & 77329.7271 & 13.5\% & 77.0\% \\
$N_3$ & 41971.8776 & 7.3\% & 84.3\% \\
$N_4$ & 26304.8502 & 4.6\% & 88.9\% \\
\bottomrule
\end{tabular}


==> tables/tab_pca_Real.tex <==
% Real curve PCA: eigenvalues and variance explained.
\begin{tabular}{llll}
\toprule
Factor & Eigenvalue & % Variance & Cumulative % \\
\midrule
$R_1$ & 137979.4380 & 68.9\% & 68.9\% \\
$R_2$ & 43459.6472 & 21.7\% & 90.5\% \\
$R_3$ & 13263.7522 & 6.6\% & 97.2\% \\
\bottomrule
\end{tabular}


==> tables/tab_pca_Spread-CDI.tex <==
% Spread-CDI curve PCA: eigenvalues and variance explained.
\begin{tabular}{llll}
\toprule
Factor & Eigenvalue & % Variance & Cumulative % \\
\midrule
$S^{CDI}_1$ & 10747.9021 & 59.5\% & 59.5\% \\
$S^{CDI}_2$ & 4117.5594 & 22.8\% & 82.4\% \\
$S^{CDI}_3$ & 2549.7595 & 14.1\% & 96.5\% \\
\bottomrule
\end{tabular}


==> tables/tab_pca_Spread-IPCA.tex <==
% Spread-IPCA curve PCA: eigenvalues and variance explained.
\begin{tabular}{llll}
\toprule
Factor & Eigenvalue & % Variance & Cumulative % \\
\midrule
$S^{IPCA}_1$ & 28781.0052 & 86.7\% & 86.7\% \\
$S^{IPCA}_2$ & 3046.2578 & 9.2\% & 95.9\% \\
$S^{IPCA}_3$ & 1357.5963 & 4.1\% & 100.0\% \\
\bottomrule
\end{tabular}


==> tables/tab_pca_Spread.tex <==
% Spread curve PCA: eigenvalues and variance explained.
\begin{tabular}{llll}
\toprule
Factor & Eigenvalue & % Variance & Cumulative % \\
\midrule
$S_1$ & 10747.9021 & 59.5\% & 59.5\% \\
$S_2$ & 4117.5594 & 22.8\% & 82.4\% \\
$S_3$ & 2549.7595 & 14.1\% & 96.5\% \\
\bottomrule
\end{tabular}


==> tables/tab_rolling_amplitudes.tex <==
% Rolling 2y-window factor amplitudes
\begin{tabular}{llrrr}
\toprule
Window start & Window end & $a^N_1$ & $a^R_1$ & $a^S_1$ \\
& & \multicolumn{3}{c}{bp/$\sqrt{\text{yr}}$} \\
\midrule
2021-01-04 & 2023-01-04 & 675 & 363 & 48 \\
2021-07-04 & 2023-07-04 & 673 & 409 & 113 \\
2022-01-04 & 2024-01-04 & 583 & 360 & 122 \\
2022-07-04 & 2024-07-04 & 554 & 341 & 134 \\
2023-01-04 & 2025-01-04 & 442 & 338 & 156 \\
2023-07-04 & 2025-07-04 & 445 & 311 & 126 \\
2024-01-04 & 2026-01-04 & 439 & 337 & 123 \\
\midrule
\multicolumn{2}{l}{Range / mean} & 43\% & 28\% & 92\% \\
\bottomrule
\end{tabular}


==> tables/tab_summary_stats.tex <==
% Summary statistics over 2021--2024, at the 3-year maturity.
\begin{tabular}{lllll}
\toprule
Variable & Mean & Std & Min & Max \\
\midrule
$f^N(t,3)$ & 11.13 & 1.43 & 7.14 & 14.33 \\
$f^R(t,3)$ & 5.79 & 1.13 & 3.05 & 8.24 \\
Breakeven $f^N - f^R$ & 5.34 & 0.66 & 2.82 & 7.53 \\
$s^{CDI}_{mkt}(t,3)$ & 182.4 & 37.7 & 125.9 & 310.9 \\
$s^{IPCA}_{mkt}(t,3)$ & 24.2 & 38.7 & -57.8 & 123.6 \\
\bottomrule
\end{tabular}


==> tables/tab_triangle_gap.tex <==
% Triangle consistency gap $\Delta(t,\tau)$: distribution across dates (bp).
\begin{tabular}{llllll}
\toprule
Maturity & Mean & Median & Std & 5th pctl & 95th pctl \\
\midrule
1y & 707.4 & 692.3 & 82.4 & 613.4 & 868.6 \\
2y & 690.8 & 677.5 & 82.7 & 578.8 & 860.9 \\
3y & 685.0 & 678.5 & 78.8 & 562.2 & 828.8 \\
5y & 694.3 & 698.8 & 56.4 & 604.4 & 791.4 \\
\bottomrule
\end{tabular}

